Demystifying a Dark Art: Understanding Real-World Machine Learning Model Development

It is well-known that the process of developing machine learning (ML) workflows is a dark-art; even experts struggle to find an optimal workflow leading to a high accuracy model. Users currently rely on empirical trial-and-error to obtain their own set of battle-tested guidelines to inform their modeling decisions. In this study, we aim to demystify this dark art by understanding how people iterate on ML workflows in practice. We analyze over 475k user-generated workflows on OpenML, an open-source platform for tracking and sharing ML workflows. We find that users often adopt a manual, automated, or mixed approach when iterating on their workflows. We observe that manual approaches result in fewer wasted iterations compared to automated approaches. Yet, automated approaches often involve more preprocessing and hyperparameter options explored, resulting in higher performance overall--suggesting potential benefits for a human-in-the-loop ML system that appropriately recommends a clever combination of the two strategies.

==> intro.tex <==
Machine learning (ML) has become a critical component of almost every domain, with users of all different levels of expertise relying on ML models to accomplish specific tasks. Developing an ML workflow can be tedious and time-consuming. Anecdotally, it may take dozens of iterations for a novice to converge on a satisfactory combination of ML model type, hyperparameters, and data preprocessing. Meanwhile, an expert might need only a small number of modifications to their original workflow to achieve comparable performance on the same task.
In such cases, novices can benefit
greatly from learning strategies employed by experts to accelerate the process of developing
effective ML workflows. With a large-scale database of user-generated workflows and evaluation scores, it becomes possible to extract aggregate workflow iteration patterns to enable this transfer of knowledge.

In this paper, we present useful insights about ML workflow development behavior of users on the OpenML\cite{Vanschoren2013} platform. OpenML is an open-source, hosted platform for users to upload datasets and run ML workflows on these datasets by calling an API. 
A relatively diverse mix of user skill levels is present on OpenML, from students just getting started with ML to experienced data scientists and ML researchers.
%Because of this, OpenML users can be thought of as a sample of all machine learning users, allowing us to generalize the results of our study as applicable for the entire machine learning community rather than specific to the OpenML platform.
OpenML publishes a database of the user-uploaded datasets as well as the workflow specifications submitted by users and their corresponding executions.
By performing targeted analyses on the most common ML models and preprocessing operators as well as their associated performance, we shed light on common ML workflow design patterns and their general effectiveness. We study trends in iterative ML workflow changes across 295 users, 475,297 runs, and 793 tasks on the OpenML platform; and draw quantitative conclusions from this crowd-sourced dataset, leading to actionable insights that help inform 
the development of future human-in-the-loop ML systems targeting novices and experts alike. 

Our main contributions can be summarized as follows:
\begin{itemize}
    \item We characterize the frequency and performance of popular ML models and preprocessing operators used by OpenML users. We highlight the impact of the operator combinations and discuss their implications on general user awareness (or lack thereof) of particular ML concepts.
    \item We analyze sequences of changes to workflows to extract different styles of ML workflow iteration and shed light on the most common types of changes for each iteration style, the amount of exploration typically performed, and performance gain users are generally able to achieve.
    \item We conduct case studies on exemplary instances to understand specific examples of both effective and ineffective iteration practices.
\end{itemize}

\textbf{Outline}. The rest of this paper is organized as follows. After a discussion of related work in Section~\ref{sec:relatedwork}, we lay out terminology and briefly explain our data processing procedure in Section~\ref{sec:method}. In Section~\ref{sec:run}, we shed light on key characteristics of the workflows commonly designed by OpenML users (at the level of individual runs). We investigate the shape and evolution of workflows across iterations as a user makes changes to improve the performance of their model for a given task in Section~\ref{sec:seq}. In Section~\ref{sec:case}, we examine case studies to give us concrete examples of effective and ineffective iterations. Finally, we present concluding insights and ideas for future work in Section~\ref{sec:conclusion}.
